HATT: Hamiltonian Adaptive Ternary Tree for Optimizing Fermion-to-Qubit Mapping

This paper introduces the Hamiltonian-Adaptive Ternary Tree (HATT) framework to compile optimized Fermion-to-qubit mapping for specific Fermionic Hamiltonians. In the simulation of Fermionic quantum systems, efficient Fermion-to-qubit mapping plays a critical role in transforming the Fermionic system into a qubit system. HATT utilizes ternary tree mapping and a bottom-up construction procedure to generate Hamiltonian aware Fermion-to-qubit mapping to reduce the Pauli weight of the qubit Hamiltonian, resulting in lower quantum simulation circuit overhead. Additionally, our optimizations retain the important vacuum state preservation property in our Fermion-to-qubit mapping and reduce the complexity of our algorithm from $O(N^4)$ to $O(N^3)$. Evaluations and simulations of various Fermionic systems demonstrate $5\sim20\%$ reduction in Pauli weight, gate count, and circuit depth, alongside excellent scalability to larger systems. Experiments on the Ionq quantum computer also show the advantages of our approach in noise resistance in quantum simulations.

==> coverletter.tex <==
\onecolumn

We thank you for your effort and constructive feedback! We have prepared the revision with the changes highlighted in blue font. Tags are added to connect the questions to the corresponding changes. Other significant changes and the answers to specific questions are listed below.

\subsection{To Reviewer A}

Thanks for your kind suggestions! We have corrected typos in our paper, and quantitative results are added to the abstract (A\#1). Here are answers to your other concerns. 

\textbf{Q1: More details on Algorithm~\ref{alg:tree-construction} and~\ref{alg:optimized-algorithm}}: We have included more explanation of both the algorithms and more step-by-step details to the provided examples (A\#2). We illustrate more figures to the example to help readers understand what happens in each step. We also clarified some explanations to reduce misunderstanding.

\textbf{Q2: Discussion of computation complexity and further reduction:} Baseline methods are Hamiltonian-dependent and thus can be prepared priorly. However, Fermion-to-qubit mapping runs only once before quantum simulation, and the generated circuit executes multiple times. Trading Fermion-to-qubit mapping complexity for lower circuit complexity is worthwhile. Besides, $O(N^3)$ is polynomial and practically allows us to scale to larger cases on classical computers. We have also added more numbers with Figure~\ref{fig:scalability} (A\#3) to show the effect of our optimization from $O(N^4)$ to $O(N^3)$. \TODO{further reduction: in each time, we can avoid iteration over all $N^3$ selections and thus reduce the complexity.}

\textbf{Q3: Discussion of when HATT is more effective and assumptions on Hamiltonians:} We added Section~\ref{sec:evaluation-discuss} (A\#4) to discuss that. Besides, we make no assumptions to Hamiltonians as they are from real physics problems.

\subsection{To Reviewer B} 

We have fixed the errors you mentioned in Section~\ref{sec:operator-pairing} (B\#2) and some more (ERR\#1). Here are other answers. 

\textbf{Q1: More discussion to Fermionic system:} We have added a paragraph in Section~\ref{sec:introduction} to discuss the importance of simulating Fermionic systems in quantum simulation (B\#1).

\textbf{Q2: More details on optimized HATT:} We have included more explanation of both the algorithms and more step-by-step information to the provided examples (B\#3). Figures show stepwise changes to the example; some descriptions are changed for better understanding.

\textbf{Q3: Whether the optimization of HATT comes at performance cost:} The optimization that reduces $O(N^4)$ to $O(N^3)$ described in Algorithm~\ref{alg:update-map} does not affect performance. It generates identical results with Algorithm~\ref{alg:optimized-algorithm}. However, operator pairing to preserve the vacuum state described in Algorithm~\ref{alg:optimized-algorithm} does generate slightly different results than Algorithm~\ref{alg:tree-construction}. The reason why we exclude comparison between the result of Algorithm~\ref{alg:tree-construction} (\textsf{unopt}) and Algorithm~\ref{alg:update-map} is that breaking vacuum state preservation makes the state preparation stage over complex. Thus lacking practical usage. \TODO{test}

\subsection{To Reviewer C} 

Thanks for the feedback! Here are the answers to your concerns. 

\textbf{Q1: Complexity in understanding:} We have added more concrete and step-by-step illustrations to the example we provided (C\#1) to help readers understand the details.

\textbf{Q2: Limited hardware testing and hardware dependency:} We have additional tested \name{} against Jordan-Wigner on multiple superconducting architectures (\textit{Manhattan}, \textit{Sycamore}, and \textit{Montreal}) with limited connectivity using a state-of-the-art circuit synthesizer Tetris~\cite{jin2024tetriscompilationframeworkvqa}. The result is provided in Table~\ref{tab:exp-extra-tetris}. \name{} still shows its advantage on end-to-end performance on these devices (C\#2).

\textbf{Q3: Generalization to other Fermionic systems:} We have conducted experiments with \name{} on several common and high-impact Fermionic systems, including electronic structures, Fermi-Hubbard model and neutrino oscillation. This proves that our method is generalized to various Fermionic systems.

\textbf{Q4: Limited comparison to optimal mapping on large scales:} To the best of our knowledge, Fermihedral~\cite{liu2024fermihedral} is the only method that generates the optimal Fermion-to-qubit mapping for \textit{specific Hamiltonian} and it does not scale due to its exponential complexity. We have already included comparing the existing prevail Fermion-to-qubit mapping on significant cases to strengthen \name{}'s advantage.

\subsection{To Reviewer D} 

Thanks for your feedback! We have corrected the symbol in Figure~\ref{fig:pauli-to-circuit}. Now the correct $\mathcal{Y}=\frac{1}{\sqrt{2}}\mqty(1 & i \\ i & 1)$ gate is shown both in the figure and also in the text description.

\subsection{To Reviewer E} 

Thanks for your review! We want to clarify the complexity of our algorithm more. Fermion-to-qubit mapping typically runs only once before quantum simulation. Thus, it is worth trading some preprocessing complexity for circuit complexity, as the circuit will run multiple times on a quantum computer. Lower circuit complexity reduces noise and hardware overhead. Besides, the $O(N^3)$ complexity allows us to generate mappings for large-scale practical Fermionic systems on classical computers. We have also included additional numbers (E\#1) in Figure~\ref{fig:scalability} to show how the reduction of complexity from $O(N^4)$ to $O(N^3)$ shortens \name{}'s time-to-solution.

\subsection{To Reviewer F}

Thanks for your feedback!

\textbf{Q1: Compared with other synthesis methods:} We have included comparisons with the circuit synthesizers you mentioned with Jordan-Wigner transformation, Rustiq~\cite{debrugière2024fastershortersynthesishamiltonian} and Tetris~\cite{jin2024tetriscompilationframeworkvqa} (on \textit{Manhattan}, \textit{Sycamore} and \textit{Montreal}), in Table~\ref{tab:exp-extra-rustiq} and~\ref{tab:exp-extra-tetris}. We discuss the result, and \name{} still shows its advantage in end-to-end performance on different synthesis methods and devices. (F\#1)

\textbf{Q2: Ideal chemistry simulation:} In the following table, we numerically solved the lowest energy eigenvalue of the Hamiltonian of $H_2$ and $LiH$ (freeze) molecules under different Fermion-to-qubit mappings to show our method does not affect the accuracy and provide scientific correctness
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}\hline
         Molecule & \sbf{JW} & \sbf{BK} & \sbf{BTT} & \sbf{FH} & \sbf{HATT} \\\hline
         $H_2$ sto3g   & -1.8573 & -1.8573 & -1.8573 & -1.8573 & -1.8573    \\\hline
         $LiH$ sto3g frz   & -1.0731 & -1.0731 & -1.0731 & -1.0731 & -1.0731    \\\hline
    \end{tabular}
    \label{tab:ideal-simulation}
\end{table}

\textbf{Q3: More benchmark details:} Details are now added to Table~\ref{tab:electronic-strcuture}. We marked the basis we used (sto3g) and whether a freeze core transformation was applied (frz/cmplt) to each molecule case.

\twocolumn
